DA-GCN: A Domain-aware Attentive Graph Convolution Network for Shared-account Cross-domain Sequential Recommendation

Shared-account Cross-domain Sequential recommendation (SCSR) is the task of recommending the next item based on a sequence of recorded user behaviors, where multiple users share a single account, and their behaviours are available in multiple domains. Existing work on solving SCSR mainly relies on mining sequential patterns via RNN-based models, which are not expressive enough to capture the relationships among multiple entities. Moreover, all existing algorithms try to bridge two domains via knowledge transfer in the latent space, and the explicit cross-domain graph structure is unexploited. In this work, we propose a novel graph-based solution, namely DA-GCN, to address the above challenges. Specifically, we first link users and items in each domain as a graph. Then, we devise a domain-aware graph convolution network to learn user-specific node representations. To fully account for users' domain-specific preferences on items, two novel attention mechanisms are further developed to selectively guide the message passing process. Extensive experiments on two real-world datasets are conducted to demonstrate the superiority of our DA-GCN method.

==> 3.3cds_graph.tex <==
\subsection{The \ac{CDS} Graph}
\noindent Given a set of sequences $S_A$ and $S_B$ in two domains of different accounts, we can model all the sequences  of two domains as a  a CDS Graph $G_{CDS}$ = (V, E), where V contains all items in two domains and all accounts appearing in the training sequences, and E contains all dependency between nodes of different three types. For example, there is a hybrid sequence $S = \left[A_1,B_1,A_2,B_2,B_3,A_3,B_4\right]$ of an account $U_1$, the detailed generation procedure of the the CDS graph is presented in Fig.2. First, we can construct two undirected account-item interaction graphs, named $G_A$ and $G_B$ respectively. Then, we can employ another two directed graphs, i.e., $G_C$ and $G_D$ to independently depict the relationship among items in domain A and domain B, respectively. Meanwhile, they can incorporate information from other sequences, as is displayed in Fig.2. Finally, we combine the four graphs as a whole CDS graph as proposed in Fig.1.
